RnGCam: High-speed video from rolling & global shutter measurements

Compressive video capture encodes a short high-speed video into a single measurement using a low-speed sensor, then computationally reconstructs the original video. Prior implementations rely on expensive hardware and are restricted to imaging sparse scenes with empty backgrounds. We propose RnGCam, a system that fuses measurements from low-speed consumer-grade rolling-shutter (RS) and global-shutter (GS) sensors into video at kHz frame rates. The RS sensor is combined with a pseudorandom optic, called a diffuser, which spatially multiplexes scene information. The GS sensor is coupled with a conventional lens. The RS-diffuser provides low spatial detail and high temporal detail, complementing the GS-lens system's high spatial detail and low temporal detail. We propose a reconstruction method using implicit neural representations (INR) to fuse the measurements into a high-speed video. Our INR method separately models the static and dynamic scene components, while explicitly regularizing dynamics. In simulation, we show that our approach significantly outperforms previous RS compressive video methods, as well as state-of-the-art frame interpolators. We validate our approach in a dual-camera hardware setup, which generates 230 frames of video at 4,800 frames per second for dense scenes, using hardware that costs $10\times$ less than previous compressive video systems.

==> Arxiv_RnGCam_2025/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\naa}[1]{\textcolor{red}{#1 -Nick}}
\newcommand{\kt}[1]{\textcolor{blue}{#1 -Kevin}}
\newcommand{\ct}[1]{\textcolor{green}{#1 -Chinmay}}


% Key variables
\newcommand{\psf}{h}
\newcommand{\xB}{\mathb{x}}
\newcommand{\rB}{\mathbf{r}}

\newcommand{\psfMat}{\mathbf{H}}
\newcommand{\cropMat}{\mathbf{C}}
\newcommand{\crop}{\text{C}}
\newcommand{\pad}{\text{P}}
\newcommand{\meas}{b}
\newcommand{\obj}{v}
\newcommand{\objVec}{\mathbf{\obj}}
\newcommand{\objVecTheta}{\mathbf{\obj}_{\theta}}
\newcommand{\measVec}{\mathbf{\meas}}
\newcommand{\Ars}{\mathbf{A}_R}
\newcommand{\Ags}{\mathbf{A}_G}
\newcommand{\UVec}{\mathbf{U}}
\newcommand{\Afull}{\mathbf{A}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{float}

==> Arxiv_RnGCam_2025/sec/0_abstract.tex <==
\begin{abstract} 
%High-speed compressive video imaging typically requires expensive capture hardware and is restricted to sparse videos with empty backgrounds. We propose RnGCam, an approach for high-speed video recovery from 20x cheaper consumer-grade rolling-shutter (RS) and global-shutter (GS) sensors. The RnGCam prototype consists of an RS sensor in conjunction with an optical diffuser. This enables capturing spatially multiplexed measurements at much higher frame rates than a standard 30 FPS sensor. We develop an implicit neural representation (INR) based method to solve the video recovery inverse problem from the captured measurements. We impose an implicit structural prior on the network, recovering the static and dynamic parts of the video separately. We show results on simulated and real data captured from our developed hardware setup, recovering 4800 frames per second (FPS) videos. We evaluate our method against modern data-driven video interpolation methods and classical total variation-based solvers, demonstrating substantial improvements.
% There has been many high-speed compressive imaging systems developed in recent years, however, most of them are limited to low background situations with high contrast, limiting its applications to controlled lab environments. Our work proposes a method to recover high speed videos by combining information from consumer-grade global and rolling shutter sensors. We propose a reconstruction method leveraging scene representations to impose an implicit factorization to seamlessly fuse the measurements together to obtain compressive high-speed video at experimental frame rates of 4,800 frames per second (theoretically up to 76,000 frames per seconds) with much more challenging background levels higher than previous methods. We experimentally test the system  complex scenes. % Compressive video capture seeks to record high-speed video using low-speed digital sensors by encoding a short video clip into a single capture, then computationally reconstructing it back. % Together, they measure complementary data: 


Compressive video capture encodes a short high-speed video into a single measurement using a low-speed sensor, then computationally reconstructs the original video. Prior implementations rely on expensive hardware and are restricted to imaging sparse scenes with empty backgrounds. We propose RnGCam, a system that fuses measurements from low-speed consumer-grade rolling-shutter (RS) and global-shutter (GS) sensors into video at kHz frame rates. The RS sensor is combined with a pseudorandom optic, called a diffuser, which spatially multiplexes scene information.
The GS sensor is coupled with a conventional lens. The RS-diffuser provides low spatial detail and high temporal detail, complementing the GS-lens system's high spatial detail and low temporal detail.
We propose a reconstruction method using implicit neural representations (INR) to fuse the measurements into a high-speed video. Our INR method separately models the static and dynamic scene components, while explicitly regularizing dynamics. In simulation, we show that our approach significantly outperforms previous RS compressive video methods, as well as state-of-the-art frame interpolators. We validate our approach in a dual-camera hardware setup, which generates 230 frames of video at 4,800 frames per second for dense scenes, using hardware that costs $10\times$ less than previous compressive video systems. 

\end{abstract}

==> Arxiv_RnGCam_2025/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

High-speed video imaging is instrumental in visualizing and analyzing fast-moving systems across disciplines, such as neuroscience~\cite{fournely2018high, lu2017video} and microscopy~\cite{zhou2023parallelized, ishijima1995high}. Conventional image sensors have limited analog-to-digital bandwidth, which limits the spatio-temporal sampling rate a given sensor can acquire. This forces a trade-off between temporal and spatial resolution. 
Conventional high-speed cameras use expensive, bulky sensors and read architectures to reduce the trade-off by directly increasing bandwidth.
%The fastest high-speed cameras can reach speeds up to 80k frames per second (find a citation). However, these devices are expensive. 

In contrast, \textit{compressive video} breaks this trade-off by encoding multiple frames of high-speed video into a single digital exposure captured with a 2D image sensor. 
The video frames are then computationally reconstructed. 
The resulting inverse problem is ill-posed and requires strong video priors to uniquely recover the video~\cite{antipa2019video, Weinberg2020100000FC}. 
% \TODO{any references that can be added to this paragraph?}

While many hardware solutions for compressive video have been proposed, we focus here on exploiting the rolling shutter (RS) available in nearly all low-cost CMOS image sensors. Previous work shows that high-speed compressive video can be recorded by coupling RS sensors with optical multiplexing elements such as diffusers \cite{antipa2019video, Weinberg2020100000FC, sheinin2018rolling}.  However, these methods rely on sparse video priors.
%and the sampled measurements at each time instant are encoded into a small row of pixels. 
As a result, they struggle to recover dense scenes with bright, detailed backgrounds. This limits their utility to relatively simple scenes with empty backgrounds, which are consistent with the sparsity priors.  
Data-driven video interpolation methods~\cite{jiang2018super,lu2022video,kalluri2023flavr} are commonly used to upsample videos captured by conventional low-fps cameras. However, since these methods are typically trained on internet videos, they often generalize poorly to out-of-distribution scenarios, particularly when interpolating chaotic motions over large temporal gaps. We demonstrate this with a simple toy experiment in~\cref{fig:toy_example_sineball}.
We aim to accelerate conventional sensors by over $100\times$, a regime in which learned upsampling performs poorly for chaotic, out-of-distribution scenes. 
\paragraph{Our Contributions:}In this paper, we address these limitations and demonstrate that RS sensors can capture high-speed compressive video of scenes comprising nontrivial backgrounds, by leveraging a few GS frames captured during the exposure of the RS sensor. We build a hardware prototype, \textit{RnGCam}, to capture optically aligned GS and RS measurements. 
% We use a differentiable forward model that fuses the GS and RS measurements. 
We propose an implicit neural representation (INR)-based space-time fusion model (STFM), to recover high-speed videos from the combination of diffuser-coded RS and GS measurements. Using GS measurements and our proposed regularization, we recover high-speed videos with dense backgrounds with much higher fidelity than previous methods~\cite{antipa2019video, 10378452}. We demonstrate our improvements over previous work, and modern data-driven video interpolators~\cite{jiang2018super, zhang2023extracting} in both simulation and on real-world data captured from \textit{RnGCam}. 
% To the best of our knowledge, this is the first demonstration of a compressive high-speed video recovery method that that our method can handle more complex scenes with denser backgrounds, demonstrating the use of a compressive high speed imaging system outside controlled lab environments.
% recover the high-speed video by We do this by fusing data from a lensless RS camera with a low-speed global shutter (GS) sensor data captured using a conventional lens.

% We do this by fusing data from a lensless RS camera with a low-speed global shutter (GS) sensor data captured using a conventional lens.


% To achieve this, we introduce a neural-space time model that accounts for static backgrounds and enables total variation regularization of the optical flow between frames. 
% \ct{This para needs re-write in the end}

% \naa{ Remove? Not sure where this sentence was going...
% show that it is possible to obtain high speed video from a diffuser coded RS measurement, while other methods such as \cite{10378452}}


% \begin{figure}[h]
%     \centering
%      \includegraphics[width=1\linewidth]{pipeline.pdf}
%     \caption{\textbf{Pipeline for fusing multiple global shutter measurements and a RS diffuser coded  long exposure measurement.} Both sensors are triggered at the same time, and in between the start and end of the RS's coded long exposure, two more images are captured as key frames using the global shutter. The RS and diffuser encodes high speed dynamics into a single measurement, and the \ct{what is a short global shutter measurement?} short global shutter measurements act as key frames for the reconstruction. The sum of a time varying and static neural scene representation is used to fuse together both measurements into a high speed reconstruction with a dense background. \TODO{font size in the figure is too small - I had to zoom to 186\% to read}}
%     \label{fig:Pipeline}
% \end{figure}



\begin{figure*}[h]
    \centering
     \includegraphics[width=1\linewidth]{figures/pipeline_camera_ready.pdf}
    \caption{\textbf{Pipeline for fusing multiple global shutter measurements and an RS diffuser coded long exposure measurement.} Both sensors are triggered at the same time, and in between the start and end of the RS's coded long exposure, two more images are captured as key frames using the global shutter. The RS and diffuser encodes high speed dynamics into a single measurement, and the GS measurements act as key frames for the reconstruction. The sum of a time-varying and static neural scene representation is used to fuse together both measurements into a high-speed reconstruction with a dense background. }
    \label{fig:Pipeline}
\end{figure*}


% In summary, \textbf{our contributions are as follows.} 
% \begin{itemize}
%     \item We propose a GS + RS diffuser capture system to achieve high-speed video in scenes with a dense background.
%     \item We develop a coordinate network-based reconstruction for compressive video. We propose an alpha blending scheme between static and dynamic networks to handle background and fuse the GS and RS measurements.
%     \item We design a hardware prototype and calibration scheme for the system utilizing two conventional GS and RS sensors.
%     \item We demonstrate high-speed reconstructions in both simulation and real measurements from prototype system for scenes that contain significant background and dense motion, outperforming similar computational imaging and data-driven interpolation for complex scenes. 
% \end{itemize}
The rest of the paper is organized as follows. We start with related work in \cref{sec:related_works}, and outline the camera model preliminaries in \cref{sec:camera_model}. We present our space-time fusion model (STFM) reconstruction algorithm in \cref{sec:neural_ST_model}. We demonstrate results on simulated and real data, and explain the RnGCam hardware setup in \cref{sec:results}.

\begin{figure}
    \centering
    \includegraphics{figures/toy_example_sineball.pdf}
    \caption{\textbf{Video interpolators struggle with complex motions.} Even with a very simple background, video interpolators produce inaccurate trajectories of the ball, with the 3 input frames at $t_1,t_2,$ and $t_3$. Our method recovers these trajectories with high fidelity.}
    \label{fig:toy_example_sineball}

\end{figure}






==> Arxiv_RnGCam_2025/sec/2_related_works.tex <==
\section{Related work}
\label{sec:related_works}
% High-speed video reconstruction using regular sensors has
% been extensively studied, with various approaches developed to overcome hardware limitations. These methods can be broadly classified into two categories. The first involves hardware modulation, either by encoding temporal information onto a conventional imaging sensor or by incorporating additional detectors, such as event cameras, to complement standard sensors. The second category relies on computational techniques, including data-driven video interpolation and neural representations, to synthesize high-frame-rate video from low-frame-rate inputs.

Methods for high-speed video recovery from regular sensors can be broadly classified into two categories. \textit{Hardware modulation} methods, which use spatial and temporal multiplexing, or capture data with additional sensors such as event cameras, to complement standard sensors. 
% has been extensively studied, with various approaches developed to overcome hardware limitations \ct{what limitations?}. 
% These methods can be broadly classified into two categories. The first involves hardware modulation, either by encoding temporal information onto a conventional imaging sensor or by incorporating 
\textit{Computational Methods}, which rely on algorithmic techniques such as data-driven video interpolation methods, or INRs to solve the inverse problem of video upsampling from compressive measurements. 

% synthesize high-frame-rate video from low-frame-rate inputs.
% Video from stills, SpinCam. Pixel wise coded exposure.


% typically leverage algorithmic techniques such as data-driven video interpolation methods, or implicit neural representations, to solve the inverse problem of video upsampling from compressive measurements. synthesize high-frame-rate video from low-frame-rate inputs.

% Dual shutter systems utilizing global and RSs have been developed for other applications such as Optical vibration sensing \cite{Sheinin:2022:Vibration}, however, there has not been a method to fuse together high-speed video from both measurements. 

% Other methods that utilize neural fields for solving inverse problems \cite{Cao2024, 9924573}

\noindent \textbf{Spatial-Multiplexing Systems:  }
Enhancing the temporal resolution of an imaging sensor can be achieved through spatial multiplexing using optical elements such as diffraction gratings or diffusers placed in front of the sensor. These elements map a single scene point to multiple sensor pixels, allowing each pixel to carry scene information across different time frames. 
Spatial multiplexing allows video recording with a limited number of pixels, reducing the bandwidth requirements. 
Different pixel arrangements have been used to subsample the sensor plane, including a single pixel \cite{duarte2008single}, a line sensor ~\cite{sheinin2020diffraction}, region of interest (ROI) ~\cite{sheinin2021deconvolving}, or a conventional RS sensor ~\cite{antipa2019video,Weinberg2020100000FC,sheinin2018rolling}. 
Because RS sensors read row-by-row, each row can encode a frame of video, increasing the frame rate by a factor proportional to the number of rows.
In all cases, reconstructing a full-frame image from limited pixel measurements is an ill-conditioned problem. 
Many of these works which rely on sparsity priors, inspired by compressed sensing, perform poorly for non-sparse scenes.  
Some work has shown improvements using INRs to enforce stronger priors, improving results significantly~\cite{monakhova2021untrained, Cao2024}.
In our work, we show that our hardware, comprising two complementary cameras, in conjunction with our INR-based video reconstruction method, produces significantly better video quality for dense scenes than previous spatial multiplexing systems. 

\noindent \textbf{Temporal-Multiplexing Systems:  }
Coding various exposures within a single frame has been widely utilized in capturing dynamic scenes to deblur the motion artifacts~\cite{holloway2012flutter}. Later, this concept was extended to reconstructing high-speed video from a single measurement ~\cite{veeraraghavan2010coded, hitomi2011video, martel2020neural, 5585094,sankaranarayanan2013compressive,iliadis2020deepbinarymask, harmany2011spatio}. 
A straightforward method is to modulate exposure time pixel-wise using a specially designed sensor that offers single-pixel exposure control~\cite{martel2020neural, iliadis2020deepbinarymask,portz2013random, willett2011compressed}.
Another approach requires dynamic optical components such as a streak camera~\cite{gao2014single}, piezoelectric stages~\cite{koller2015high, liu2018rank,llull2013coded}, spatial light modulator (SLM)~\cite{hitomi2011video,sankaranarayanan2013compressive, reddy2011p2c2} or digital micromirror device (DMD)~\cite{deng2019sinusoidal,wang2017compressive} to generate different designed patterns at a higher time rate to encode the temporal information. 
These specialized optical components and sensors are expensive and have a limited frame rate. 
Additionally, many of the methods struggled in non-sparse scenes~\cite{sheinin2021deconvolving, sheinin2020diffraction}.
Our method uses a homemade diffuser made of optical epoxy on cover slides, while still allowing us to recover frame rates of up to $4800$ with a single calibrated PSF image.

\noindent \textbf{Multi-Sensor systems:}
Another common approach is combining multiple sensor types to compensate for the limitations of a single sensor. Event cameras, valued for dynamic sensitivity, capture information missed by regular RGB sensors~\cite{tulyakov2021time, tulyakov2022time, zhang2024event}. However, they are expensive, saturate with camera motion, and Timelens \cite{tulyakov2021time} requires training with a large video-event dataset, and reports at most 15 frame skip compared to our 130. Similarly, camera arrays have achieved high-speed video capture~\cite{wilburn2005high}. Other works have fused RS and GS for video recovery without optical multiplexing, recovering video with relatively low frame rates ~\cite{fan2021inverting}. Integrating consumer-grade GS and RS sensors to collect complementary data is an innovative approach to decoding high-speed information~\cite{Sheinin:2022:Vibration}, though it has not been directly applied to video recovery. Building on this idea, our method inserts a diffuser in front of the RS to encode dynamic information instead of a speckle pattern while using a standard RGB sensor to preserve high-frequency details.
% Our method similarly requires two detectors to provide complementary information, but utilizes commercially available, low-cost sensors.

\noindent \textbf{Data-driven video frame interpolation methods:  } Our work closely relates to video frame interpolation (VFI), a well-studied computer vision problem ~\cite{parihar2022comprehensive}. Popular VFI methods use convolution- or transformer-based models with implicit architectural priors and are trained on large datasets. Recent works predict frames as discrete time steps given a start and end frame \cite{Li_2023_CVPR, kalluri2023flavr, niklaus2017video, lu2022video}. In contrast, ours enables continuous frame interpolation along the time axis. We hence compare our work with the popular method SuperSlomo~\cite{jiang2018super}, and more recent work EMA-VFI~\cite{zhang2023extracting}, which allow continuous time interpolation between frames. Our approach outperforms these methods (see \cref{sec:results}), without being trained on large datasets.

% Given a start and end frame,~\cite{, etc} predict intermediate frames at discrete time steps, while ~\cite{jiang2018super, }rely on convolution or transformer architectures 

% Video interpolation methods \cite{zhang2023extracting, jiang2018super, jin2023unified}

\noindent \textbf{Implicit Neural Representations (INRs) for inverse problems:  }
Coordinate-based neural networks have been gaining popularity for a variety of visual computing tasks, for a full survey, refer to \cite{10.1111:cgf.14505}. Our work closely relates to approaches~\cite{Cao2024, 9924573,9606601} that use INRs in computational imaging inverse problems. In our paper, we adopt SIRENs \cite{DBLP:journals/corr/abs-2006-09661} as our signal representation. A variety of other neural representations have been developed with different architectures to increase the representation ability of these coordinate networks \cite{Saragadam_2023_CVPR,lindell2021bacon, Xie_2023_CVPR}.

==> Arxiv_RnGCam_2025/sec/3_method.tex <==
\section{Fusing GS and coded RS images to handle complex scenes}
\label{sec:camera_model}

In an optical system that utilizes spatio-temporal multiplexing optics like ours, there is a finite amount of information that can be encoded into a single measurement. This is particularly apparent in complex scenes with stronger backgrounds, where the background signal is mixed and aggregated with the signal of interest and makes the recovery of the dynamic portion of the signal much more challenging. 

As illustrated in Figure \ref{fig:Pipeline}, our system consists of two sensors aimed at the same scene by utilizing a beam splitter to divide the light equally between the coded RS arm and the arm with the GS sensor at imaging conditions.

In this section, we first present the acquisition scheme for our data capture. We then illustrate the image formation model for the coded RS image and GS images.
% and our proposed method of using neural scene representations to fuse all the collected data to obtain reconstructions with significantly more challenging scenes than previous methods.
Our goal in this paper, is to exploit the RS behavior to gain access to the data that GS would miss in the long gaps between frames, while using the high quality GS images, imaged with a conventional lens, to improve the spatial detail of the recovered high-speed video.  
%\naa{Summarize our goal is to recover video from GS and RS measurements}
\subsection{General camera model}
Here we describe the model for a general sensor combined with an optical system with a known shift-invariant PSF, $h(\xi,\eta)$. Assuming no occlusions, the time-varying intensity arriving at the sensor from a dynamic scene $\obj(\xi,\eta,\tau)$ is given by 2D linear convolution
\begin{equation}\label{eq:linear_conv}
    \widetilde{\obj}(\xi,\eta,\tau)=\obj\left(\xi,\eta,\tau\right)\stackrel{(\xi, \eta)}{*}h(\xi,\eta),
\end{equation}
where $\stackrel{(\xi,\eta)}{*}$ denotes 2D convolution over the continuous spatial dimensions $(\xi,\eta)$, for time $\tau$.  We discretize the problem onto grid $(x,y,t)$ and approximate \eqref{eq:linear_conv} as
% \begin{equation}\label{eq:discrete_2D_conv}
%     \widetilde{\obj}[i,j,k] = \crop \left[ \pad \left( \psf[i,j] \right) \stackrel{(i,j)}{\circledast} \pad \left( \obj[i,j,k]\right ) \right]
% \end{equation}
\begin{equation}\label{eq:discrete_2D_conv}
    \widetilde{\obj}(x,y,t) = \crop \left[ \pad \left( \psf(x,y) \right) \stackrel{(x,y)}{\circledast} \pad \left( \obj(x,y,t)\right ) \right]
\end{equation}
where $\circledast$ is circular convolution, $\pad$ operator is 2D zero padding, and $\crop$ is 2D cropping such that $\crop(\pad(v)) = v$. 
Note that our optical system includes a field stop which limits the support of the scene to an area strictly smaller than the sensor, which is why $\obj$ can be zero-padded in \eqref{eq:discrete_2D_conv}. Finally, the digital measurement recorded by a sensor is 
\begin{equation}\label{eq:general_exposure}
    \meas(x,y) = \sum_t S(x,y,t)\widetilde{\obj}(x,y,t){,}
\end{equation}
where $S(x,y,t)$ is an indicator that encodes the sensor's exposure timing at pixel $(x,y)$, taking on value 1 when a pixel is actively recording photons, and 0 otherwise. Substituting \eqref{eq:discrete_2D_conv} into \eqref{eq:general_exposure} yields a general camera model for a system with a known PSF and sensor exposure pattern. In subsequent sections, we describe $S$ and $h$ for each of our two cameras. 

\subsection{Rolling and Global shutter timings}
%
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/shutter_timing_camera_ready.pdf}
    \caption{\textbf{Shutter timing diagram.} Blue depicts active RS rows, and red depicts active GS rows. $T^R_e$ is the exposure time for a single RS row, $\tau_\text{line}$ is the lag time between rows, and $T^G_e$ is the exposure time for the GS. At $T_0$, a long RS exposure is triggered, and 3 short GS exposures are triggered at $T^{G}_1$, $T^{G}_2$, and $T^{G}_3$. %\textbf{b)} Point spread function of rolling shutter sensor obtained by shining point source into system.
    }
    \label{fig:timing_diagram}
\end{figure}
%
%
%
The timing diagram in Figure \ref{fig:timing_diagram} shows a comparison between global and rolling shutter sensors. The rolling shutter exposes each row of pixels for the same exposure time, $T_{e}^R$ with a short delay, $\tau_{\mbox{line}}$, in the onset of exposure as compared to the previous row. We represent this as the indicator function, \(S_R(x,y,t)  =  \mbox{rect}\left(\frac{1}{T_e^R}\left[t - y\cdot \tau_{\mbox{line}}\right]\right)\).
%of width $T_e^R$ and row-dependent delay $y \cdot \tau_{\mbox{line}} + T_e^R/2$.
The delay between rows is typically very short, on the order of microseconds, whereas 
global shutter has a relatively long gap between exposures due to pixel readout.



%the acquisition scheme we use to collect data. RS sensors expose a subset of the rows at each time. Each row is exposed for $T^R_\text{row}$ and after a short delay of $T^R_l$, the next row is exposed. Between the start and end of the RS exposure ($T_0$ and $T^R_e$), three short GS exposures at time $T_0$, $T_M$, $T^R_e$, where all the pixels in the sensor are exposed, are taken as an estimate for the key-frames \TODO{(cite someone here)}.

\subsection{Rolling shutter and Diffusers}
%\begin{figure}
%    \centering
    %\includegraphics[width=1\linewidth]{ICCV2025-Tandi-Submission/GSRS_diffuser_conv_explainer.pdf}
    %\caption{\textbf{Lensless camera forward model}. The intensity recorded at a lensless camera sensor is the 2D convolution of the diffuser PSF $\psf$ and the scene $\obj$.}
    % The intensity arriving at the sensor of a lensless camera is described by 2D convolution between the diffuser PSF, $\psf$, and the scene, $\obj$.}
    %\label{fig:diffuser_2d_conv}
%\end{figure}
The RS arm comprises an RS sensor and a smooth, pseudorandom phase optic called a diffuser. The diffuser maps each scene point to a large, structured PSF, $\psf$.  The intensity arriving at the sensor, $\widetilde{\obj}(x,y,t)$, from an extended scene $\obj(x,y,t)$ is described by convolution~\eqref{eq:discrete_2D_conv}. As illustrated in Figure \ref{fig:diffuser_RS_GS}(a), the large PSF spreads scene information over the entire sensor, which plays a critical role in enabling high-speed video using rolling shutter.

% For a dynamic 2D scene, the spreading of information The A 2D scene, $\obj(x,y)$, The PSF of our camera is shown in Figure \ref{fig:diffuser_2d_conv}. As shown in \cite{antipa2019video}, this large, structured PSF spreads information about all scene points into each row of pixels, enabling the RS read-out to see the entire scene at every time point. 

% \naa{Paragraph and fig explaining diffusercam visually. Mention sparse scenes are OK (cite) and dense is not (refer to figure). Be sure to introduce $h_R(x,y)$, the caustics, and point to figure. $h_R$ will be used in fig}. 

%\begin{figure}
 %   \centering
    %\includegraphics[width=1\linewidth]{ICCV2025-Tandi-Submission/GSRS_measurement_explainer.pdf}
   % \caption{\textbf{Illustrating the capture process of a dynamic scene.} 
    % Our RS-diffuser camera (top) and GS-lens camera (bottom). 
 %   \textit{Left}: The scene is a red ball moving sinusoidally in the $y-$direction. The RS-diffuser camera (\textit{top}) measurement $\meas_{R}$, records the dynamic intensity, $\tilde{\obj}$ distributed all over the sensor due to convolution with the large diffuser PSF. This encodes rich spatio-temporal information in $\meas_{R}$ about the entire scene. The GS-lens camera (\textit{bottom}) acquires three 2D images, trading temporal information for better spatial detail than the RS-diffuser. This motivates our system design wherein we fuse the two measurement types into a high-speed video.}
%    \label{fig:meas_explainer}
%\end{figure}

% Illustration of the capture process of a dynamic scene
% using an RS-diffuser camera (top) and GS-lens camera (bot-
% tom). The scene (left) is a red ball moving sinusoidally in the
% y−direction. After convolution with the large diffuser PSF, the
% dynamic intensity, ˜v, at the sensor is distributed everywhere. Af-
% ter acquisition with the RS sensor, the final RS-diffuser measure-
% ment, bR, contains rich spatio-temporal information about the en-
% tire scene. In this example, the GS-lens camera (bottom) acquires
% three 2D images. While this method loses temporal information,
% it has better spatial detail than the RS-diffuser and does not suf-
% fer from 2D deconvolution noise. This motivates our system de-
% sign wherein we fuse the two measurement types into a high-speed
% video.

%An RS sensor exposes each row for the same duration, $T_e^R$. The onset of each row's exposure is delayed by $\tau_{\mbox{line}}$ from the row preceding it. As a result, the RS shutter indicator function, $S_R$, is described by a temporal rectangle function of width $\T_e^R$ and row-dependent delay $y \tau_{\mbox{line}} + T_e^R/2$. 

% Because each row's exposure window is delayed by $\tau_\text{line}$ seconds from the row preceding it, the rolling shutter problem naturally has a temporal grid with spacing of $\tau_\text{line}$ (i.e., $t = k \tau_\text{line}$). With this in mind, each pixel's exposure time is $W_k^R = T_\text{e}^R/\tau_\text{line}$ time points long, with its start delayed by one time point from the previous. The discretized RS shutter function is thus described by $S_R[k|j] = \mbox{rect}\left(\frac{k - j}{W_k^R} - \frac{1}{2}\right)$. Note that we typically downsample $S$ onto a smaller grid as discussed in \naa{where is this discussed?}. 

The process of capturing a dynamic scene with a diffuser and RS sensor is illustrated in Figure \ref{fig:diffuser_RS_GS} (c). The single 2D measurement recorded by the RS-diffuser camera, $\meas_R$, is described by substituting $S_R$ and $h$ into~\eqref{eq:discrete_2D_conv} and~\eqref{eq:general_exposure}.  %and is visualized in the top right of Figure \ref{fig:meas_explainer}. 
Because the diffuser distributes the scene intensity values in a structured way over the entire sensor, the $\meas_R$ contains information about nearly all spatial points at each time during RS acquisition. As shown in prior work \cite{antipa2019video, Weinberg2020100000FC}, this enables recovery of sparse video from RS-diffuser measurements. However, these approaches struggle with dense scenes (Fig. \ref{fig:simulation_results} (d) and (e)). We denote the RS-diffuser measurement process for a video with $M \times N$ spatial samples and $K$ frames in matrix-vector form as 
\begin{equation}\label{eq:RS_matrix_form}
    \measVec_R = \Ars \objVec
\end{equation}
where $\Ars: \mathbb{R}^{MNK} \mapsto \mathbb{R}^{MN}$ is the matrix form of \eqref{eq:general_exposure}, $\measVec \in \mathbb{R}^{MN}$ and $\objVec\in\mathbb{R}^{MNK}$ are column-stacked versions of $\meas$ and $\obj$, respectively. The details of $\Ars$ are in \cref{supp:matrix_details}.
%\cite{antipa2019video}. 
%\naa{We need to connect $\mathbf{A}_R$ to \eqref{eq:general_exposure}. Something like "$\mathbf{A}_R$ is the matrix representation of the linear model in \eqref{eq:general_exposure} with the shutter function being 1 during active exposure and 0 otherwise as illustrated in \ref{fig:timing_diagram}; see supplement section BLAH for detail" Then in supplement say the full definition of $S$ using rectangle functions (see video from stills paper)}
% \naa{NOTE: We need to update all math in the supplemental derivations to match notation here!!}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=1\linewidth]{figures/GSRS_diffuser_explainer_merged.pdf}
    \caption{ \textbf{Lensless camera forward model}. (\textit{a}) The intensity arriving at a lensless camera sensor is the 2D convolution of the diffuser PSF $\psf$ and the scene $\obj$.     
     \textbf{Illustrating the capture process of a dynamic scene.} All $y$-$t$ images are slices aligned with the ball's $x$-coordinate.
      (\textit{b}) The scene is a red ball moving sinusoidally in the $y$-direction. The RS-diffuser camera (\textit{c}) measurement $\meas_{R}$, records the dynamic intensity, $\tilde{\obj}$ distributed all over the sensor due to convolution with the large diffuser PSF. This encodes rich spatio-temporal scene information into $\meas_{R}$. The GS-lens camera (\textit{d}) acquires three 2D images, trading temporal information for better spatial detail than the RS-diffuser. This motivates our system design wherein we fuse the two measurement types into a high-speed video. 
     }
    \label{fig:diffuser_RS_GS}
\end{figure*}

\subsection{Global shutter and lens}
The global shutter sensor is coupled with a high quality lens, so we assume its PSF is $h_G(x,y) \approx \delta(x,y)$. However, the lens does have some distortion, and the magnification is not the same as the RS camera, so we perform a coordinate transform on the measurements as described in \cref{supp:coordinate_alignment}.  This allows us to model the intensity arriving at the GS sensor as approximately equal to the scene, $\obj(x,y,t)$. 
In our implementation, we capture three GS exposures at times $T_1^G$, $T_2^G$, and $T_3^G$, spanning the RS capture time. The GS shutter function for the $l-$th GS capture is given by $S_G^l(t) = \mbox{rect}\left(\frac{1}{T_e^G}\left[t - T_l^G\right] \right)$. As illustrated in Figure \ref{fig:diffuser_RS_GS}(d), the combination of GS exposure and a lens produces three frames containing full 2D scene information at the instants the GS sensor was triggered. Note that the GS sensor is blind for most of the video duration due to its slow readout time. The GS measurements are described by
\begin{equation}
    b_G^l(x,y) = \sum_t S_G^l(t) \obj(x,y,t){.}
\end{equation}
We denote in matrix-vector form as
\begin{equation}
    \measVec_G^l =  \Ags^l  \objVec
\end{equation}
where $\Ags^l : \mathbb{R}^{MNK} \mapsto \mathbb{R}^{MN}$ is the matrix describing GS exposure model and $\measVec_G^l$ is the column-stacked version of the $l-$th GS measurement. The collection of all 3 GS measurements, as a vector $\measVec_G \in \mathbb{R}^{3MN}$, is given by
\begin{equation}
    \measVec_G = \Ags \objVec
\end{equation}
where $\Ags = [(\Ags^1)^\intercal|(\Ags^2)^\intercal|(\Ags^3)^\intercal]^\intercal$ is the combined forward model of the three GS captures. Our goal is to compute a high-speed video containing hundreds of frames given only the four frames captured by our two systems: one RS-diffuser capture, and three GS-lens images. With the camera models described above, the high-speed video can be estimated by solving the optimization problem:
\begin{equation}
\label{eq:inverse_problem}
    \widehat{\objVec} = \arg\min_\objVec \|\Afull \objVec -   \measVec\|_2^2
\end{equation}
where $\Afull = \left[\Ags^\intercal | \psi \Ars^\intercal\right]^\intercal$ is a matrix modeling both cameras, and $\measVec = \left[\measVec_G^\intercal |\measVec_R^\intercal \right]^\intercal$ contains all four measured frames in vector form. The parameter $\psi\geq 0$ controls the weight given to the RS measurements. This formulation fuses the GS and RS measurements, allowing us to use GS measurements for estimating 
the spatially high-frequency components of the scene, and RS measurements for temporal frame upsampling. 

This problem is highly underdetermined, so strong video regularization is required to recover the correct video uniquely. While prior work~\cite{antipa2019video} applies 3D total variation (3DTV) on the grid $\mathbf{v}$ as a regularizer, we propose a space-time fusion model (\cref{sec:neural_ST_model}) that allows explicitly regularizing spatio-temporal consistency. 


% which is more memory efficient than optimizing over the entire memory grid, and also is more flexible in terms of imposing a stronger regularization strategy.

% \ct{Can we define the inverse problem here itself? Coz here v is already a grid.}
% \ct{And then later we introduce the coordinate MLP notations, and talk about that in more detail. And then we can add another version of the equation, (currently eq.7) with the MLP modifs.}
% We use a short shutter speed to obtain 3 different measurements of the scene to be used as key-frames in the reconstruction at times . Since the global shutter arm is at imaging condition, we can model it approximately as 
% \begin{equation}
%     b^1_G =\mathbf{I}I_1
% \end{equation}

% Where $\mathbf{I}$ is the identity matrix. We denote the 3 global shutter images we obtain at time $T_0, T_M $ and $T^R_e$ as $b_G^1, b_G^2, $ and  $b_G^3$.




\section{Space-Time Fusion Model Reconstruction}
\label{sec:neural_ST_model}
% Our proposed neural space-time model (STFM) represents the video using INRs.  
Our proposed space-time fusion model (STFM) leverages two intrinsic properties of high-speed videos\textemdash static-dynamic decomposition and local spatiotemporal consistency. STFM explicitly factorizes the video into an alpha blend of static (background) and dynamic (foreground) components. Each video component is modeled with a separate INR, see \cref{fig:SIREN_explainer}. We also explicitly model a motion-warping field with a separate INR to locally regularize the spatio-temporal motion in the video. These inductive biases in our design alleviate the ill-posedness of the inverse problem in \eqref{eq:inverse_problem} and significantly improve the reconstruction. We demonstrate this through ablation in \cref{sec:ablations}. We first briefly overview INRs followed by an explanation of our proposed STFM. 

% High-speed videos have smooth spatial motion between adjacent frames due to the high frame rate. we also to incorporate high-speed video-specific priors, such as using s inductive biases in the network architecture. 

% \cref{subsec:recon_alg}.
% In \cref{subsec:hardware} we outline the RnGCam hardware setup we built to capture the measurements for solving the high-speed video inverse problem.
% \naa{As Gal has suggested, we should motivate the model here. Something about wanting to capture movement of foreground objects, blend them with background, and have access to flow fields for regularization purposes.}
% explain our developed hardware capture setup 



% \subsection{Reconstruction Algorithm}
% \label{subsec:recon_alg}
\noindent \textbf{Implicit Neural Representations:  }
%INRs are neural networks $F_{\theta}:\mathbb{R}^{P}\mapsto\mathbb{R}^{Q}$ with parameters $\theta$ that approximate a function $f:\mathbb{R}^{P}\mapsto\mathbb{R}^{Q}$ which maps from $P$-dimensional input to a $Q$-dimensional signal (e.g., a scalar field or RGB values). When used as coordinate neural networks, they can be trained such that 
INRs are neural networks $F_{\theta} : \mathbb{R}^{P} \to \mathbb{R}^{Q}$, with parameters $\theta$, that provide a continuous approximation to a target function $f : \mathbb{R}^P \to \mathbb{R}^Q$ defined on a $P$-dimensional input domain and producing a $Q$-dimensional signal (e.g., a scalar field or RGB values). When used as coordinate neural networks, they can be trained such that $F_{\theta}(\gamma(\mathbf{x})) \approx f(\mathbf{x}), \forall \mathbf{x}\in \mathbb{R}^{P}$
% \begin{equation}
%      \label{eq:INR}
%     F_{\theta}(\gamma(\mathbf{x})) \approx f(\mathbf{x}), \forall \mathbf{x}\in \mathbb{R}^{N}
%  \end{equation}
where $\mathbf{x}$ is the coordinate vector and $\gamma(\cdot)$ denotes the commonly used positional encoding function~\cite{mildenhall2020nerf}, defined in \cref{supp:space-time_fusion}. For brevity we denote $F_{\theta}(\gamma(\mathbf{x}))$ as $F_{\theta}(\mathbf{x})$ in the rest of the text. In our work, we use SIREN~\cite{martel2020neural}, an INR with sinusoidal activations as the representation backbone for our neural space-time model.

%
\begin{figure*}[ht!]
    \centering
    % Placeholder for figure
    \includegraphics[width=1\linewidth]{figures/SIREN_explainer_camera_ready.pdf}
    \caption{\textbf{Space-Time Fusion Model for compressive video}. Both rolling and global shutter measurements are used to simultaneously update both static and dynamic networks by computing their loss against the estimated measurements from querying the estimated scene $\mathbf v_{\theta}$ and passing it through the optical forward model, $A$.  
    % \textbf{b) Example outputs from motion $F^{M}_{\theta}$},  
    % \textbf{c) Alpha channel of dynamic SIREN $F^{D}_{\theta}$},  
    % \textbf{d) RGB channel of dynamic SIREN $F^{D}_{\theta}$},  
    % \textbf{e) RGB channel of static SIREN $F^{S}_{\theta}$}.  
    $F^{D}_{\theta}$ takes in a grid of spatiotemporal coordinates while $F^{S}_{\theta}$ only takes in a grid of spatial coordinates. The two outputs are summed together after the alpha map is applied.}
    \label{fig:SIREN_explainer}
\end{figure*}
%

\noindent \textbf{Space-Time Fusion Model:  }
We explicitly decompose the video into its static and dynamic components using two separate INRs, $F_{\theta}^S$ and $F_{\theta}^{D}$, respectively, as shown in \cref{fig:SIREN_explainer}. While INRs are continuous functions, our data is measured on a discrete spatiotemporal grid. We therefore evaluate the INRs on a spatiotemporal coordinate tensor $\mathbf{X} \in \mathbb{R}^{MNK\times3} =\left[\mathbf{X}^{xy}, \mathbf{X}^{t}\right]$, where $\mathbf{X}^{xy}\in\mathbb{R}^{MNK\times 2}$ contains the spatial coordinates $(x,y)$ and $\mathbf{X}^{t}\in\mathbb{R}^{MNK \times 1}$ contains the temporal coordinate $t$. We adopt the notation \( F(\mathbf{X}) \) to denote row-wise evaluation: each row of \( \mathbf{X} \) is treated as an input to \( F \). Note that the grid structure arises from the discrete pixel structure of the sensor. More details on $\mathbf{X}$ are in the \cref{supp:space-time_fusion}.

To evaluate the final video color $\mathbf{v}_{\theta}\in \mathbb{R}^{MNK\times 3}$ on the full grid $\mathbf{X}$, we first compute the background RGB color $\mathbf{v}^{S}_{\theta}\in \mathbb{R}^{MNK\times 3}$, which remains constant over time for each spatial location. This is done by evaluating the static INR $F^{S}_{\theta} : (x,y)\mapsto (R,G,B)$ on the spatial grid: $\mathbf{v}^{S}_{\theta} = F^{S}_{\theta}(\mathbf{X}^{xy})$. 
% \\
% $$
To capture the motion of the dynamic component, we predict a \textit{time-varying} motion warp field  $\mathbf{U}(t)\in \mathbb{R}^{MNK\times2}$ using the motion INR $F^{M}_{\theta}: (x,y,t)\mapsto (u_x(t), u_y(t))$,
 \begin{equation}
\label{eq:motion_network_pred}
    \mathbf{U}(t) = [\mathbf{U}_x(t), \mathbf{U}_y(t)] =F^{M}_{\theta}(\mathbf{X}), 
\end{equation}
where $\mathbf {U}_x(t), \mathbf {U}_y(t) \in \mathbb{R}^{MNK}$ denote the time-varying \(x-\) and \(y-\)direction spatial offsets of the grid $\mathbf X$, respectively.

To compute the dynamic color $\mathbf{v}^{D}_{\theta}(t)$, and transparency $\boldsymbol{\alpha}_{\theta}(t) \in [0,1]$, we first \textit{warp} the spatial input grid $\mathbf X^{xy}$ with the motion field $\mathbf U(t)$. The dynamic INR $F^{D}_{\theta} : (x,y) \mapsto (R,G,B,\alpha)$ is then queried as follows: 
 \begin{equation}
    \left[\mathbf{v}^{D}_{\theta}(t), \boldsymbol{\alpha}_{\theta}(t)\right] = F^{D}_{\theta}(\mathbf{X}^{xy}+ \mathbf{U}(t)).
\end{equation}

% The input to the dynamic INR $F^{D}_{\theta} : (x,y) \mapsto (R,G,B,\alpha)$
% is \textit{warped} using $\mathbf U$ to capture dynamic motion. $(x,y)$ is spatially offset using a time-varying motion warp field 
% $\mathbf{U} =[\mathbf {U}_x, \mathbf U y]\in\mathbb{R}^{MNK\times 2}$, which is predicted using the motion INR $F^{M}_{\theta}: (x,y,t)\mapsto (u_x, u_y)$ as
%  \begin{equation}
% \label{eq:motion_network_pred}
%     \mathbf{U} = [\mathbf{U}x, \mathbf{U}y] =F^{M}_{\theta}(\mathbf{X}). 
% \end{equation}



% \TODO{can you elaborate a bit more here? the mention of the warp field is very out of the blue} %\ct{done}
% also should it be U_x and U_y, ie using subscripts?

The final video is a composite of the static and dynamic colors and is computed as %\TODO{we haven't motivated why we have $\alpha$ - what are we gaining from this? what would have happened if we didn't have $\alpha$ and the output was just the sum of static and dynamic recovery} 
%\ct{done}
\begin{equation}
    \label{eq:final_video}
    \mathbf{v}_{\theta} = \boldsymbol{\alpha}_{\theta}(t)\mathbf{v}^{S}_{\theta} + (1-\boldsymbol{\alpha}_{\theta}(t))\mathbf{v}^{D}_{\theta}(t).
\end{equation}
Alpha compositing the static and dynamic components with a time-varying $\alpha$ helps account for occlusions in STFM. 

\noindent \textbf{Inverse problem:  }
The high-speed video recovery inverse problem in~\eqref{eq:inverse_problem} can now be expressed as
\begin{equation}
    \widehat{\theta} = \arg\min_\theta \|\Afull \objVecTheta -   \measVec\|_2^2
\end{equation}
where we solve for the INR parameters $\theta$ instead of directly optimizing for the spatio-temporal grid. The high-speed video can then be recovered using~\eqref{eq:final_video} with the optimized INR parameters $\widehat{\theta}$. Please see \cref{supp:space-time_fusion} for details.

\noindent \textbf{Regularization:  }
% Previously, methods utilizing 3DTV priors on the scene \cite{8747341, 7745938} struggle to regularize dense scenes. \citet{cao2022dynamic} shows the effectiveness of neural spacetime models for imaging inverse problems. 
% Additionally, explicit motion modeling in this method allows regularizing local motion dynamics, which we describe in Eq. \eqref{eq:loss_function}.
We explicitly model spatial warping through the motion network, regularizing its output $\mathbf{U}$ (we drop $(t)$ for brevity) with anisotropic total variation: 
\begin{equation}
\label{eq:TV_anisotropic}
    \text{TV}_S(\mathbf{U}) = \|\mathbf{U}_x\|_\text{TV} + \|\mathbf{U}_y\|_\text{TV},
\end{equation} where  $\|\cdot\|_\text{TV}$ is the anisotropic 3D total variation semi-norm with temporal weighting factor $\beta$ defined as 
\begin{equation*}
    ||\UVec||_\text{TV} = \sum_{x,y,t} |\nabla_x \UVec| + |\nabla_y \UVec| + \beta |\nabla_t \UVec|, \UVec \in \mathbb{R}^{M\times N \times K}
\end{equation*}
Note that $\mathbf{U}$ is reshaped back to the spatio-temporal grid resolution, before applying anisotropic TV. 
Regularizing the motion fields constrains local dynamics, and significantly improves the reconstruction quality for dense scenes, as demonstrated in \cref{fig:simulation_results}. In comparison, previous works~\cite{antipa2019video,kamilov2017TV} that directly apply 3DTV on the grid $\mathbf{v}$ struggle to regularize dense scenes. 
The resulting optimization objective on incorporating the motion field TV regularization~\eqref{eq:TV_anisotropic}, is given as 
\begin{equation}
\label{eq:invpo}
\begin{aligned}
    % \mathcal{L}, ~~\textrm{where}\\ 
     \widehat{\theta} &= \arg\min_\theta \left\{ \|\Afull \objVecTheta -   \measVec\|_2^2 + \tau \text{TV}_S(\mathbf{U})\right\}.
    \end{aligned}
\end{equation}
% \begin{align}
% \label{eq:final_loss}
%     \mathcal{L}=\|\Ags \objVecTheta -   \measVec_G\|_2^2 + \psi \|\Ars \objVecTheta - \measVec_R\|_2^2 + \tau TV_S(\mathbf{U}).
% \end{align}
For experimental data, we slightly modify \eqref{eq:invpo} to also optimize for the relative white balance between the GS and RS measurements, see \cref{supp:coordinate_alignment} for details. 
We defer the implementation details, including the hyperparameters $\tau,\beta, \psi$, and INR architecture in the \cref{supp:prototype detail}.  

% \subsection{RnGCam Hardware Setup}
% \label{subsec:hardware}
% %\TODO{BLAH BLAH}

% % \noindent \textbf{Hardware Setup:}
% We designed and built the RnGCam prototype, (\cref{fig:experimental_setup}), illustrated in \cref{fig:Pipeline}. 
% Our setup utilized a relay optical system and a 90/10 beam splitter followed by a primary lens to simultaneously collect the same scene using rolling shutter with diffuser and global shutter with lens.
% We use a set exposure time $T^G_e, T^R_e $ of GS and RS sensors to $650 \mu s$. Our RS sensor has a line time of $13 \mu s$. 
% Due to memory limitations for the coordinate network grid, we downsample our working grid by $16$ in space and time, resulting in an effective line time of $208 \mu s$ ($4,807$ fps).
% Details about the prototype implementation can be found in ~\cref{supp:prototype detail}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=8cm]{figures/experiment_setup_camera_ready.pdf} % Adjust width as needed
    \caption{\textbf{RnGCam Experimental Setup.} 
    \textit{Right:} RnGCam hardware consists of an RS arm (RS sensor and optical diffuser)and the GS arm (GS sensor and lens). We use a beam splitter supplemented with relay optics to ensure optical consistency between the two arms. All these components are placed inside a light-tight box.
    \textit{Left:} PSF captured for the RS arm.}
    % \textit{Left} is the captured PSF for the RS arm of the system. Right shows the experimental setup consisting of the main lens, relay optics, beam splitter, RS sensor with a diffuser, and a global shutter sensor with a lens. }
    \label{fig:experimental_setup}
    \vspace{-12pt}
\end{figure}
%\TODO{do you want to briefly mention timing here- otherwise I think that detail is mentioned in the abstract, and then buried in the appendix}
 
% \noindent \textbf{System timing:  }
% We use a set exposure time $T^G_e, T^R_e $ of GS and RS sensors to $650 \mu s$. Our RS sensor has a line time of $13 \mu s$. 
% Due to memory limitations for the coordinate network grid, we downsample our working grid by $16$ in space and time, resulting in an effective line time of $208 \mu s$ ($4,807$ fps). 
% The downsampling factor of 16 in space and time was chosen because of a combination of memory limitations and the very high resolution of the RS sensor. 
% Because our effective frame rate is limited by the downsampling we have to fit the coordinate network to our machine (48GB NVIDIA A40), a lower resolution RS sensor with a similar line time could get us to around $77,000$ fps.


% $TV_s = \sum_{x,y,t} |\Delta_x V_x| + |\Delta_y V_x| + \beta |\Delta_t V_x| + |\Delta_x V_y| + |\Delta_y V_y| + \beta |\Delta_t V_y|$
% To solve the above inverse problem in 
% Fusing the global shutter measurements $\mathbf{b}_{G}$
% Fusing the three global shutter measurements, $\mathbf{b}_{G}$ $[b_G^1, b_G^2, b_G^3]^T$, and one long exposure from the diffuser-coded RS measurement, $b_R$, allows us to use global shutter measurements as an estimate for the spatially high-frequency components of the scene, while using the RS measurement to estimate the frames in between.

% To achieve this, we propose a reconstruction method illustrated in \cref{fig:SIREN_explainer} using a coordinate neural scene representation. A coordinate neural network takes in inputs in the form of coordinates $\mathbf{r} = (x,y,t)$ as shown in \cref{fig:SIREN_explainer} a. These coordinates are then fed into the model composed of multi-layer perceptrons (MLPs). Specifically, we use the SIREN \cite{DBLP:journals/corr/abs-2006-09661} network architecture. 

% The first module, the motion network $F^M_\theta$, takes in spatiotemporal coordinates $(x, y, t)$ and outputs a time-motion field denoted by $(\Delta x(t), \Delta y(t)$).  This is summed with the input grid coordinates, resulting in $(x + \Delta x(t), y +\Delta y(t)$) visualized in \cref{fig:SIREN_explainer}(b) as $\widehat{I}_M(x,y,t)$. $\widehat{I}_M(x,y,t)$ is taken as an input for the module $F^{D}_{\theta}$ which predicts the dynamic RGB channels, $\widehat{I}_D(x,y,t)$\ shown in Figure \ref{fig:SIREN_explainer}(d), and alpha blending channel $\alpha(x,y,t)$, illustrated in Figure \ref{fig:SIREN_explainer}(c). 
% % \ct{$\Delta$ has been used as pixel size before. It's being used as difference in positions here above.}
% Finally, another network $(x,y)$, denoted as static SIREN,  $F^{S}_{\theta}$, takes in a subset of the coordinate grid at time $0$ to produce a static estimate to the scene, $\widehat{I}_S(x,y,t)$ shown in Figure \ref{fig:SIREN_explainer} (d). The full representation can be written as:
% \begin{equation}
% \begin{split}
% F_{\theta}(x,y,t) &= \alpha(x,y,t) \cdot F^{D}_{\theta}(F^M_\theta(x,y,t)) \\
% &\quad + (1-\alpha(x,y,t)) \cdot F^{S}_{\theta}(x,y, 0)
% \end{split}
% \end{equation}
% where, as shown in Figure \ref{fig:SIREN_explainer} (a), $x, y, t \in G(x,y,t)$ is the input coordinate grid containing the 3D spatiotemporal coordinates used to query the coordinate networks.

% We apply a non-negativity constraint on both the static and dynamic networks, and apply a sigmoid to keep the alpha channel between 0 and 1. 

% This structure results in an implicit factorization in the reconstruction that is the sum of a static background component and a time varying component. This is illustrated in an example scene in Figure \ref{fig:SIREN explainer}.b. As a result of this implicit factorization, we are able to utilize the global shutter measurements as an estimate for the static background, while estimating dynamic components using the RS measurements. We demonstrate this through simulation and real world experiments in Section \ref{sec:results}.

% We chose to use a multi-layer perceptron scene representation as they have been shown to regularize 3D volume reconstructions well compared to a voxel-based representation ~\cite{mildenhall2020nerf, 10.1111:cgf.14505}. \ct{this is not correct, the citation as well isn't correct / relevant here.}


% \begin{equation}
% \label{eq:pos_enc}
% \gamma(\mathbf{r}) = (\mathbf{r}, \cos{(2^i\pi \mathbf{r})}, \sin{(2^i \pi \mathbf{r})}, \dots) \text{, for } \textit{i} = 0, \dots, l-1
% \end{equation}, 
% where $l$ is a tunable parameter.

% By having one time-varying representation output a dynamic $(x,y,t)$ scene and another static representation output static $(x,y)$ image, we are able to also cleanly integrate measurements from both sensors. 
% \subsection{Inverse problem}
% Now that we have formulated a scene representation, we solve for the scene by minimizing the loss with respect to the model parameters, $\theta$. 
% A sampled video, 
% %\ct{replace (x,y,t) with $\mathbf{X}$ in the equations below where X denotes a $N\times3$ vector of all points in the space-time grid.}
% \begin{equation}
% \begin{split}
% \underset{\theta}{\arg\min} \, \mathcal{L} = \|\Ags F_{\theta}(x,y,t) - \measVec_G \|_2^2 + \\
% \psi \|\Ars F_{\theta}(x,y,t) - \measVec_R\|_2^2 + \tau\|\nabla_{xyt}F^M_\theta\|_1
% \end{split}
% \label{eq:loss_function}
% \end{equation}
% % where $\Ags$ and $\Ars$ are the forward models associated with the GS and RS cameras, respectively. The operator $\nabla_{xyt} = [\nabla_x, \nabla_y, \beta\nabla_t]^T$ computes the finite forward differences in $x$, $y$, and $t$ for the motion field, $F^M_\theta$, and $\beta$ is an additional weight the temporal total variation sparsity. (We found that $\beta$ values from 10 - 10000 yielded the best results, depending on the scene). \naa{We need to mention that we don't actually flatten and use matrix-vector multiplies. Everything has different dimensions in code, but we use the linear algebra notation only for the equations in the paper.}

% The estimated measurements are used to compute the mean squared error with $b_G$ and $b_R$ and we minimize this loss with respect to the parameters of the coordinate networks. We minimize this using the Adam optimizer with learning rate 0.5e-5. 
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/simulation_results_camera_ready.pdf}
    \caption{\textbf{Comparing our reconstruction with competing methods on a complex scene.} a) A simulated scene of a smoke plume emerging from a gun barrel (credit: \href{https://www.youtube.com/watch?v=dpr4a89YzE8}{The Slow Mo Guys} ). We compare our method with video interpolators and 3DTV-based methods by calculating PSNR over the entire video. The video interpolators (red inset) b) EMA-VFI \cite{zhang2023extracting} and c) Super SloMo \cite{jiang2018super} fail to recover information present early in the video in the intermediate frames, as they only rely on key-frames (GS) and thus are prone to hallucination. d,e) 3DTV-based methods resolve these details due to the presence of coded RS measurements but have poor reconstruction quality. f) Our method resolves intermediate details with a significantly higher fidelity. We also achieve the highest PSNR calculated over the full video.}
    \label{fig:simulation_results}
\end{figure*}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/psnr_comparison_all_methods.pdf}
    \caption{\textbf{Comparing per-frame PSNR for all methods}. Video interpolators achieve high PSNR near the three input GS frames (start, mid, end) indicated by the black vertical lines, but show degradation for intermediate frames. Our method is more temporally stable, achieving the highest PSNRs on intermediate frames (excluding GS frames). We show results on the scene in \cref{fig:simulation_results}, with the stars corresponding to the estimated frames in \cref{fig:simulation_results}.  
    \vspace{-18pt}
    }
    \label{fig:psnr-perframe}
\end{figure}

==> Arxiv_RnGCam_2025/sec/4_experimental_setup.tex <==



==> Arxiv_RnGCam_2025/sec/5_implementation.tex <==
%\section{Implementation}
%\label{sec:implementation}



% We present the prototype of the system in Fig.~\ref{fig:experimental_setup}. 
% The system uses global- and rolling-shutter cameras to capture the same scene simultaneously through a primary lens followed by a relay optical system with a beam splitter at the conjugate plane. 

% The primary lens is a Sigma 50mm EX DG HSM Lens with f-number 1.4, and a field stop is set at the focal plane to control the field of view.
% Then, two 2-inch 98 mm focal length doublets with effective focal lengths around 45 mm collimate the light and image the aperture of the primary lens to a physically accessible plane where the diffuser will be located to avoid vignetting.
% The distance between the two doublets' last surface and the pupil's image is designed to be sufficient to fit in a 1 inch visible light beam splitter, which has 90/10 uneven energy distribution. 
% The RS arm requires more energy because of spatial multiplexing. 
% Therefore, the higher intensity arm has a 1" format RS camera (Basler ace acA5472-17uc, IMX183) with a diffuser containing random microlenses with a 9/16-inch radius and an effective focal length of around 28mm. 
% The weaker intensity arm of the beam splitter has one 1/1.2" format global shutter camera (Basler ace acA1920-155uc, IMX174) with a Fujinon 25mm 1.4 f-number machine vision lens to form the static reference image. 

% A function generator syncs cameras with a hardware trigger to start simultaneously, triggering the subsequent three global shutter frames between a RS frame. 


% \subsection{Prototype and implementation}
% We present the prototype of the system in Fig.~\ref{fig:experimental_setup}. 
% The system uses global- and rolling-shutter cameras to capture the same scene simultaneously through a primary lens followed by a relay optical system with a beam splitter at the conjugate plane. 
% The primary lens is a Sigma 50mm EX DG HSM Lens with f-number 1.4, and a field stop is set at the focal plane to control the field of view.
% Then, two 2-inch 98 mm focal length doublets with effective focal lengths around 45 mm collimate the light and image the aperture of the primary lens to a physically accessible plane where the diffuser will be located to avoid vignetting.
% The distance between the two doublets' last surface and the pupil's image is designed to be sufficient to fit in a 1 inch visible light beam splitter, which has 90/10 uneven energy distribution. 
% The RS arm requires more energy because of spatial multiplexing. 
% Therefore, the higher intensity arm has a 1" format RS camera (Basler ace acA5472-17uc, IMX183) with a diffuser containing random microlenses with a 9/16-inch radius and an effective focal length of around 28mm. 
% The weaker intensity arm of the beam splitter has one 1/1.2" format global shutter camera (Basler ace acA1920-155uc, IMX174) with a Fujinon 25mm 1.4 f-number machine vision lens to form the static reference image. 

% A function generator syncs cameras with a hardware trigger to start simultaneously, triggering the subsequent three global shutter frames between a RS frame. 


% \noindent \textbf{PSF calibration:  }
% The point spread function of the system, $h$, shown in Figure \ref{fig:experimental_setup} (a) is experimentally obtained by shining a point light source to the main lens of the system shown in \cref{fig:timing_diagram}
%  b).


==> Arxiv_RnGCam_2025/sec/6_results.tex <==
\section{Results}
\label{sec:results}

In this section, we compare the performance of our method relative to video interpolators and 3DTV \cite{antipa2019video} in simulation, and demonstrate our reconstructions at 4,800 fps on real experimental data obtained from our hardware prototype.

% Details on system timing, PSF calibration, and the optical setup are provided in the supplemental section.

\subsection{Simulation results}
We compare our reconstructed results with several data-driven video interpolators \cite{zhang2023extracting, jiang2018super, jin2023unified} and reconstruction with 3D total variation (3DTV) regularization adopted by previous papers \cite{antipa2019video, Weinberg2020100000FC} in \cref{fig:simulation_results}, for a scene with complex motion patterns. 
% \TODO{Citations not compiling here}. 
We use the 3 GS frames as input for the video interpolators and solve for 60 intermediate frames. For the single and dual shutter 3DTV reconstructions, the inputs are the spatially multiplexed rolling shutter measurements. Classical TV-based methods perform poorly for scenes with dense backgrounds due to the lack of strong motion and smoothness priors see~\cref{fig:simulation_results}.
Video interpolators tend to perform better or comparable to our method on scenes that resemble their training data, such as simple and sparse motion like in~\cref{fig:bird} with a natural image background. For more complex motions (\cref{fig:simulation_results}), we outperform all the baselines. The combination of high-frame-rate RS measurements with STFM regularization enables our method to accurately recover intermediate frame details in scenes with complex motion. 
In \cref{sec:ablations}, we include ablations to examine the contributions of different components of both the STFM model and our measurements.




\begin{figure*}
    % \centering
    \includegraphics[width=1\linewidth]{figures/Experimental_results_camera_ready.pdf}
    \caption{\textbf{Experimental results from our hardware setup.} We show the 3 GS  (\textit{left}) and RS measurements (\textit{middle}) for each scene. We show a subset of the 231 reconstructed frames (\textit{right}) at $4807$ Hz. We recover the static and dynamic components with high fidelity.}
    \label{fig:exp-real}
\end{figure*}

\subsection{RnGCam Hardware Setup}
\label{subsec:hardware}
%\TODO{BLAH BLAH}

% \noindent \textbf{Hardware Setup:}
We designed and built the RnGCam prototype, (\cref{fig:experimental_setup}), illustrated in \cref{fig:Pipeline}. 
Our setup utilized a relay optical system and a 90/10 beam splitter followed by a primary lens to simultaneously collect the same scene using RS with diffuser and GS with lens.
We use set exposure times $T^G_e, T^R_e $ of GS and RS sensors to $650 \mu s$. Our RS sensor has a line time of $13 \mu s$. 
Due to memory limitations for the coordinate network grid, we downsample our working grid by $16$ in space and time, resulting in an effective line time of $208 \mu s$ (4,807 fps).
Details about the prototype implementation are in ~\cref{supp:prototype detail}. In contrast to previous RS-diffuser works ~\cite{antipa2019video}, our setup does not require a dual shutter sCMOS camera, which costs $>\$20k$ USD, and produces better results.
\subsection{Experimental results}
In Figure \ref{fig:exp-real}, we demonstrate the ability of our prototype to resolve high-speed dynamics with a dense background component. We record a scene of a spinning propeller with a checkered background (top), and a scene of a tennis ball being caught by a hand, with complex background (bottom) containing high-frequency details, e.g., the zebra. 

Our method temporally resolves the spinning propeller (\cref{fig:exp-real}, top row), while simultaneously estimating and blending the occluded color checker in the background with the propeller blades. We also resolve the motion of the tennis ball together with the complex background scene (\cref{fig:exp-real}, bottom row). In \cref{fig:3dtv_exp}, we show that 3DTV performs poorly on the start frame due to the time-varying field of view \cite{antipa2019video}; intermediate frames also contain strong artifacts and poor detail.


\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/3DTV_experimental.pdf}
    \caption{\textbf{3DTV failure with single shutter}. 3DTV for a single shutter (\textit{top}) fails at early  frames due to blind spots. Reconstructions at intermediate frames still contain artifacts. In contrast, our method (\textit{bottom}) recovers these frames at high fidelity.}
    \label{fig:3dtv_exp}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/ablation_bird_camera_ready.pdf} % Adjust width as needed
    \caption{\textbf{Failure Case.} We recover high-frequency details better than 3DTV-based methods, but video interpolators perform comparably (SuperSloMo) or better (EMA). This is expected since video interpolators are well suited for scenes with sparse and simple motions, such as the shown bird wing flap (credit: \href{https://www.youtube.com/watch?v=iVKdU_OmsaU}{SmarterEveryDay}).} \vspace{-12pt}
    \label{fig:bird}
\end{figure}





% \subsection{Comparison with video intepolators}


% \begin{figure}[h]
%     \centering
%     % Placeholder for figure
%     \rule{8cm}{6cm} % Width = 10cm, Height = 6cm
%     \caption{Compare with video interpolators?}
%     \label{fig:large_diffuser}
% \end{figure}

% Compare with FLAVR video intepolation 



==> Arxiv_RnGCam_2025/sec/7_limitations.tex <==
\section{Limitations}
\label{sec:limitations}
We assume the capture setup to be static, and that the scene can be factorized into a static background and dynamic foreground. 
Our proposed STFM relies on a warping assumption to model inter-frame motion. As a result, it struggles with scenes where objects appear suddenly, violating the spatio-temporal consistency assumption. We use SIREN in SFTM, using more recent video-specific INRs~\cite{Saragadam_2023_CVPR} might further improve video reconstruction quality. SFTM fits to all data, and GS frames are not hard constraints.

Our method requires scenes to be well-lit due to the RS-Diffuser sensor's low light throughput, caused by the diffuser's large sensor footprint. We are limited by GPU memory constraints and the small pixel size of commercially available rolling shutter sensors, restricting us to lower spatial and temporal resolutions. In the absence of these constraints, our method can theoretically achieve $77,000$ fps. 
% We are downsampling-limited due to GPU memory constraints and a small pixel size of commercially available rolling shutter sensor. Without downsampling the spacetime grid induced by the rolling shutter, we can theoretically hit a frame rate close to $77,000$ fps.
% light due to the narrow exposure band, leading to low SNR. % \naa{finish}
%, so there can be improvements made, such as modeling the scene representation as a more expressive low rank + sparse representation \cite{7439735}. Regarding the signal representation of our coordinate network, we have yet to explore other methods with spatially compact activations~\cite{Saragadam_2023_CVPR}, which can help with resolving higher frequencies in the reconstructions. 

% Further work can improve on the model to handle these types of scenes. 
% Our current representation can only handle a specific class of scenes with a non-time-varying background. We also assume that there is no camera motion, further exploration of scenes with camera motion is needed.  In future work, We can expand to model camera motion.

% Additionally, due to the object full scene being encoded to just a few sensor rows, small, low contrast objects in dense scenes are hard to recover. 

% A

% Compared to 3DTV, this method allows us to explicitly regularize the flow field, enabling more targeted regularization. More exploration can be done to regularize these flow fields using motion field-specific regularizers~\cite{6951417}.



==> Arxiv_RnGCam_2025/sec/8_future_work.tex <==
\section{Conclusion}
\label{sec:conclusion}
We demonstrated compressive high-speed video recovery at an effective frame rate of $4.8$ kHz with a dual camera setup consisting of low-cost consumer-grade sensors.  
Our prototype \textit{RnGCam} is 10x cheaper than existing compressive video recovery setups~\cite{antipa2019video}. 
RnGCam consists of an RS-diffuser arm that captures high temporal detail and a GS arm that captures high spatial detail. 
Fusing these complementary measurements lets us recover high-speed videos with dense backgrounds. 
Previous methods rely on much more expensive hardware but still fail in this scenario. 
For fusing GS-RS measurements, we proposed an INR-based space-time fusion model, which explicitly imposes static-dynamic factorization on the video and also models spatio-temporal warping.
These inductive biases significantly improve the quality of our recovered high-speed videos. 
We evaluate our method on simulated and real data captured with RnGCam. 
We outperform an existing computational imaging method ~\cite{antipa2019video} and also demonstrate superior performance over data-driven video interpolators for scenes with complex motion. 

\newpage
\noindent\textbf{Acknowledgements} This work was supported by a Kavli Institute for Brain and Mind Innovative Research Grant. 

% spatial measurements through the global shutter and lens, and high and a rolling shutter sensor with a diffuser. sensors of fusing global and spatially multiplexed rolling shutter measurements using dynamic and static coordinate networks to obtain high-speed video. Our experimental prototype utilizes low-cost sensors with conventional rolling shutter architecture and achieves an effective frame rate of $4,806$ Hz. With the addition of a global shutter sensor, we are also able to reconstruct videos with much denser backgrounds while previous methods were only able to work with sparse scenes with a dark background. We show results from our method on simulated and experimental data that our method outperforms similar computational imaging methods, and also demonstrate superior performance over data-driven video interpolators in more complex scenes. 







